Sampling of Shape Expressions

Cyber-physical systems (CPS) are increasingly becoming driven by data, using multiple types of sensors to capture huge amounts of data. Extraction and characterization of useful information from big streams of data is a challenging problem. Shape expressions facilitate formal specification of rich temporal patterns encountered in time series as well as in behaviors of CPS. In this paper, we introduce a method for systematically sampling shape expressions. The proposed approach combines methods for uniform sampling of automata (for exploring qualitative shapes) with hit-and-run Monte Carlo sampling procedures (for exploring multi-dimensional parameter spaces defined by sets of possibly non-linear constraints). We study and implement several possible solutions and evaluate them in the context of visualization and testing applications.

==> 2stages.tex <==

\subsection{A two-stage semantics for shape expressions}
\label{sec:twostep}
In the sampling procedure proposed here, it is important to produce not only signals, 
but also information about why they match the given shape expression. 
There are two reasons why a signal matches an expression: 
first, it follows a sequence of atomic shapes (hereafter called  shape words) that agrees with the definition of the shape expression;
second, the parameter valuation that enables the matching satisfies the constraint.

The first stage of the semantics of a shape expression $\f$ is given as the set of shape words $\swsem{\f}$ defined above.

We now describe the second stage: from a shape word to parameter valuation and then noiseless signals. 
For a constraint $\gamma$, we denote by $\ParamSet(\gamma)$ the set of parameter valuations $v$ that satisfies $\gamma$, 
that is $\ParamSet(\gamma)=\{v \mid v \models \gamma\}$. 
Further, we assume that every constraint $\gamma$ involved in this paper yields a set $\ParamSet(\gamma)$ 
whose volume is well-defined and non-null.  
%\textcolor{red}{REMOVE and SPEAK OF MEASURABLE FUNCTION WHEN DEFINING CONSTRAINTS,
%and assume that it is measurable (that is its volume is well-defined) for every constraint $\gamma$ involved in $\varphi$.} 
Given a shape word $u$, every parameter valuation $v \in \ParamSet(\gamma)$  maps to a signal
$\valtosig{u}{\gamma}(v)$ \todo{$w_{u,v}$ would make more sense! What do we mean by $w_{u,\gamma(v)}$... Normally, our signals depend on X and t. Here, we craft a signal from $u$ and $v$.} with parameters of the atomic shapes instantiated with $v$.
\begin{definition}[Semantic of a shape word]
The noiseless language of a shape word $u$ and a constraint $\gamma$ is the set  
$\L_0(u,\gamma)=\{(\valtosig{u}{\gamma}(v),v)\mid v\in \ParamSet(\gamma)\}$. %which is included in $\L_0(\varphi).$
\end{definition}

\todo{Here I wrote a new para, we can merge it with the beginning of the next section}
The sampling procedure we describe next follows two stages:
(1) first, a shape word is randomly chosen, and 
(2) a parameter valuation satisfying the constraint of this shape word is randomly chosen so that a signal is created. 
The two stages will be uniform but we do not guarantee uniformity for the overall distribution. 
This notion is in fact ill-defined, since two shape words of the same length do not require the same number of parameters.

==> garbage-collector.tex <==

\begin{theorem}\label{theorem:prop}
\begin{enumerate} 
\item The word sampler is a Boltzmann sampler~\cite{boltzmann-sampling}, that is 
(1a) it can uniformly sample words of different size; (1b) it can uniformly sample words with a given average size; (1c) it is uniform for every possible size of output sample, {\em i.e.} every two words of the same size have the same probability to be chosen.
\item Let $(u,\gamma)$ be a shape word selected by the word sampler. Let $v_k$ denote the parameter valuation satisfying the constraint $\gamma$ sampled by the point sampler after $k$ steps. Let $w_k$ be the signal corresponding to the shape word $u$ and parameter valuation $v_k$. Then, 
\begin{itemize} 
\item (2a) The probability of sampling $u$ is $\displaystyle Prob(u)=\frac{z^{|u|}}{g_{\f}(z)}}$, where $g_{\f}(z)$ is the generating function computed by Algorithm~\ref{alg:genfun} and $z$ is a parameter chosen depending on the expected length of $u$ as in Remark~\ref{remaek:root}. 
\item (2b) Let $\NoiselessSignalSet_{\varphi}(u, \gamma)$ be the set of noiseless signals corresponding to the shape word $(u, \gamma)$ which is assumed to have nonzero volume. For any nonzero-volume set $U \subseteq \NoiselessSignalSet_{\varphi}(u, \gamma)$ and any given value $\epsilon > 0$, there exists $K_{\epsilon}$ such that $|Prob(w_{K_{\epsilon}} \in U) - vol(U)/vol(\NoiselessSignalSet_{\varphi}(u, \gamma))| < \epsilon$.
\end{itemize}
\end{enumerate}
\end{theorem} 
\begin{itemize}
\item 
$\swsem{\epsilon}=(\epsilon,\top)$, 
    \item 
$\swsem{a}=(a,\top)$, 
    \item 
$\swsem{\varphi_1\cup\varphi_2}=\swsem{\varphi_1}\cup \swsem{\varphi_2}$,   
\item 
%$\swsem{\varphi_1 \cdot 
%\varphi_2}=
%\{(u_1 \cdot u_2,\gamma_1\wedge \gamma_2) \mid \, (u_i,\gamma_i)\in S(\varphi_i), i \in \{ 1, 2 \} \, \}$, 
$\swsem{\varphi_1 \cdot 
\varphi_2}=\swsem{\varphi_1}\cdot\swsem{\varphi_2}$
%\{\alpha_1.\alpha_2 \mid \, \alpha_1\in \swsem{\varphi_1}, \alpha_2\in \swsem{\varphi_2} \, \}$, 
\item 
$\swsem{\varphi^*}=\cup_{i\geq 0} \swsem{\varphi^i}$ %=\{(u_1\cdots u_n,\wedge_{i=1}^n\gamma_i)\mid (u_i,\gamma_i)\in \swsem{\varphi}, i \in \{ 1, \ldots, n \} \, \}$,
\item 
$\swsem{\f:\gamma}=(\epsilon,\gamma)$.
\end{itemize}


==> oldSElanguage.tex <==
The semantics of SE is defined in terms of a \emph{language} $\L$.
\begin{definition}[SE language] \label{def:noisySE}
    The language $\L$ of a shape
    expression is defined as follows:
    \begin{align*}
        \L(\epsilon) &= \{ (w,v) \st |w| = 0 \} \\
        \L( f(x, p_{1}, \ldots, p_{n}, \dvar)) &= \{(w,v) \st |w| = v(\dvar) \text{ and } w(x) = f(x)[p_{1}\backslash v(p_1), \ldots, 
        p_{n}\backslash v(p_n)] \}\\
        \L(\psi_1 \cap \psi_2) &= \L(\psi_1) \cap \L(\psi_2) \\
        \L(\f_1 \cdot \f_2) &= \{(w_1 \cdot w_2, v) \st (w_1,v) \in \L(\f_1) \text{ and } (w_2,v) \in \L(\f_2) \} \\
        \L(\f_1 \cup \f_2) &= \L(\f_1) \cup \L(\f_2) \\
        \L(\f^*) &= \bigcup_{i=0}^\infty \L(\f^i) \\
        \L(\f : \gamma) &= \{ (w,v) \st (w,v) \in \L(\f) \text{ and } v \models \gamma \}
    \end{align*}
\end{definition}
A signal $w$ is in the language if (1) $w$ can be segmented 
into a sequence of atomic shapes defined by SE, and (2) for 
each atomic shape in the sequence there exists a parameter valuation 
under which the observed segment and the 
instantiated atomic shape are the same.


==> ztmpops.tex <==
\font\zmsy=zmsy10

%% Define Temporal Operators

\newcommand\cir{\mathop{\hbox{\zmsy\char'062}}}
\newcommand\dia{\mathop{\hbox{\zmsy\char'061}}}
\newcommand\boc{\mathop{\hbox to 11truept{\hfill\zmsy\char'060\hfill}}}

\newcommand\cirM{\mathop{\hbox{\zmsy\char'023}}}
\newcommand\diaM{\mathop{\hbox{\zmsy\char'121}}}
\newcommand\boxM{\mathop{\hbox to 11truept{\hfill\zmsy\char'140\hfill}}}

\newcommand\until{\hskip 1.5pt\hbox{$\cal U$}\hskip 0.5pt}
\renewcommand\unless{\hskip 1.5pt\hbox{$\cal W$}\hskip 0.5pt}
\newcommand\since{\hskip 1.5pt\hbox{$\cal S$}\hskip 0.5pt}
\newcommand\backto{\hskip 1.5pt\hbox{$\cal B$}\hskip 0.5pt}
\newcommand\ent{\hbox{\hskip 1.5pt\hbox{$=$\hskip
-3pt\hbox{$\succ$}\hskip 0.5pt}}}

\newcommand\Next{\cir}
\newcommand\X{\cir}
\newcommand\sU{\until}
\newcommand\wU{\unless}
\newcommand\sS{\since}
\newcommand\wS{\backto}
\newcommand\DiamondM{\diaM}
\newcommand\Previous{\cirM}
\newcommand\BoxM{\boxM}
\newcommand\G{\boc}
\newcommand\F{\dia}
\newcommand\opH{\boxM}
\newcommand\opP{\diaM}
\newcommand\XX{\Next}
\newcommand\Y{\Previous}
\newcommand\YY{\Previous}
\newcommand\ssU{\unless}
\newcommand\Sscr{\since}
\newcommand\fildia[1]{\opP}
\newcommand\filcir[1]{\Y}
\newcommand\filboc[1]{\opH}
\newcommand\wY{\filcir{\sim}}
\newcommand\emm[1]{\mbox{\em #1\/}}
%\newcommand\true{\emm{True}}
%\newcommand\false{\emm{false}}

